Few-shot Medical Image Segmentation with Cycle-resemblance Attention

Recently, due to the increasing requirements of medical imaging applications and the professional requirements of annotating medical images, few-shot learning has gained increasing attention in the medical image semantic segmentation field. To perform segmentation with limited number of labeled medical images, most existing studies use Proto-typical Networks (PN) and have obtained compelling success. However, these approaches overlook the query image features extracted from the proposed representation network, failing to preserving the spatial connection between query and support images. In this paper, we propose a novel self-supervised few-shot medical image segmentation network and introduce a novel Cycle-Resemblance Attention (CRA) module to fully leverage the pixel-wise relation between query and support medical images. Notably, we first line up multiple attention blocks to refine more abundant relation information. Then, we present CRAPNet by integrating the CRA module with a classic prototype network, where pixel-wise relations between query and support features are well recaptured for segmentation. Extensive experiments on two different medical image datasets, e.g., abdomen MRI and abdomen CT, demonstrate the superiority of our model over existing state-of-the-art methods.

==> 6_Supplementary_Materials.tex <==
\section*{Supplementary Material}


\noindent\textbf{Qualitative Results of Experiments in \textit{setting 2}.} 
In order to further demonstrate the visual segmentation results of both settings, we also show some qualitative results under \textbf{\textit{setting 2}} on both datasets in Figures.~\ref{suppct} and~\ref{suppmri}.
As can be seen, for the abdominal CT dataset, our proposed method makes a segmentation that covers most of the \textit{liver} area, while the result of SSL-ALPNet only covers half of the \textit{liver}.
Moreover, the segmentation results of SSL-APLNet have visible false positive volumes for the examples in \textit{left kidney}, \textit{right kidney} and \textit{spleen}, while our method makes segmentation which are closed to the ground truth for those 
\begin{figure}[H]
\centering
\includegraphics[width=1\linewidth]{Figures/suppct.pdf}
   \caption{The qualitative results under \textbf{\textit{setting 2}} on abdominal-CT dataset.}
\label{suppct}
\end{figure}
\noindent classes. For the abdominal MRI dataset, our method performs a better segmentation of the class \textit{spleen} and \textit{liver} than that of the SSL-ALPNet. 
Last, our segmentation result of \textit{left kidney} and \textit{right kidney} aligns closer to the ground truth class boundary than results of SSL-ALPNet does.
Therefore, our approach makes a more precise segmentation especially on drawing the boundary of the classes.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{Figures/suppmri.pdf}
   \caption{The qualitative results under \textbf{\textit{setting 2}} on abdominal-MRI dataset.}
\label{suppmri}
\end{figure}


\begin{table}[H]
\centering
\begin{tabular}{cccccc}
\toprule
\# of Blocks     & LK             & RK             & Spleen         & Liver          & Mean           \\ \midrule
1                & 80.39          & 82.42          & \textbf{74.52} & 71.93          & 77.30          \\
3                & \textbf{82.45} & 85.06          & 72.16          & 75.94          & 78.90          \\
5                & 81.95          & \textbf{86.42} & \textbf{74.32} & \textbf{76.46} & \textbf{79.79} \\
7                & 82.08          & 83.93          & 73.35          & 73.16          & 78.13          \\
9                & 80.27          & 83.93          & 73.61          & 74.28          & 78.02          \\
12               & 82.41          & 85.84          & 71.88          & 73.02          & 78.29          \\
15               & 80.71          & 86.00          & 73.88          & 72.67          & 78.31          \\ \bottomrule
\end{tabular}
\caption{Experiments results (in Dice Score) on the number of Cyc-Resemblance blocks on abdominal MRI in \textit{\textbf{setting~1}}.}
\label{supblocks}
\end{table}

\begin{algorithm*}[h] \small
    \PyFunc{def} \PyCode{ \textsc{cra}(sup\_ft, qry\_ft, num\_block):} \PyComment{Cycle-Resemblance Attention Module}\\
    \PyCode{~~~~init\_sup\_ft = sup\_ft.detach().clone()} \PyComment{copy initial support feature}\\
    \PyCode{~~~~init\_qry\_ft = qry\_ft.detach().clone()} \PyComment{copy initial query feature}\\
    \PyCode{~~~~for n in range(num\_block):}\\
    \PyCode{~~~~~~~~sup\_ft = \textsc{update\_ft}(sup\_ft, init\_qry\_ft)} \PyComment{Update the support feature}\\
    \PyCode{~~~~~~~~qry\_ft = \textsc{update\_ft}(qry\_ft, init\_sup\_ft)} \PyComment{Update the query feature}\\
    \PyFunc{~~~~return} \PyCode{sup\_ft, qry\_ft} \\
    
    \PyFunc{def} \PyCode{\textsc{update\_ft}(ft\_A, ft\_B):} \PyComment{Returns the updated feature A}\\
    \PyCode{~~~~g\_ft\_A = g(ft\_A)} \PyComment{g is a $1\times 1\times 1$ torch.nn.Conv2d layer}\\
    \PyCode{~~~~phi\_ft\_A = phi(ft\_A)} \PyComment{phi is a $1\times 1\times 1$ torch.nn.Conv2d layer}\\
    \PyCode{~~~~theta\_ft\_B = theta(ft\_B)} \PyComment{theta is a $1\times 1\times 1$ torch.nn.Conv2d layer}\\
    \PyCode{~~~~ftA\_flat = torch.flatten(ft\_A)} \PyComment{flatten the feature tensor}\\
    \PyCode{~~~~ftB\_flat = torch.flatten(ft\_B)} \\
    \PyCode{~~~~affine = ftA\_flat @ ftB\_flat.transpose()} \PyComment{Matrix mult.; A as row, B as col}\\ 
    \PyCode{~~~~ftA2ftB\_idx = affine.max(dim=column)[1]} \PyComment{col index with max value for each row}\\
    \PyCode{~~~~ftB2ftA\_star\_idx = affine.max(dim=row)[1]} \\
    
    \PyCode{~~~~}\PyComment{find the most resemble pixel $i^*$ of pixel $i$ in feature A }\\
    \PyCode{~~~~}\PyComment{via cycle resemblance operation}\\
    \PyCode{~~~~ftA2ftA\_star\_idx = torch.gather(ftA2ftB\_idx, ftB2ftA\_idx)} \\
    \PyCode{~~~~ftA\_star\_flat = torch.gather(ftA\_flat, ftA2ftA\_star\_idx)} \\
    
    \PyCode{~~~~}\PyComment{cosine similarity between pixel $i$ and $i^*$ for each $i$ in feature A}\\
    \PyCode{~~~~similarity = torch.nn.CosinSimilarity(ftA\_flat, ftA\_star\_flat)}  \\
    \PyCode{~~~~wt = torch.nn.softmax(similarity)} \PyComment{softmax} \\
    \PyCode{~~~~wt = wt.reshape()} \PyComment{unflatten}\\
    
    \PyCode{~~~~y = g\_ft\_A * wt} \\
    \PyCode{~~~~W\_y = W(y)} \PyComment{W is a $1\times 1\times 1$ torch.nn.Conv2d layer}\\
    \PyCode{~~~~z = ft\_A + W\_y} \\
    \PyFunc{~~~~return} \PyCode{z}
\caption{Pseudo code of Cycle-Resemblance Attention in PyTorch-like style.}
\label{algo:cra}
\end{algorithm*}

\noindent\textbf{Number of Attention Blocks.}
Additionally, to establish a more complementary sensitive analysis on the influence of the number of attention blocks, we conduct the experiment where the number of Cyc-Rsemblance blocks is set as $3$ on abdominal-MRI dataset under \textbf{\textit{setting 1}}.
All experimental results are shown in Table.~\ref{supblocks}, from which we can draw the same conclusion as we did in the main paper, where the optimal performance can be achieved when the number is set as $5$, and stacking multiple attention blocks has a beneficial effect on segmentation performance, while the excessive amount of blocks can also do harm to the model, making the network pay much attention on local details and thus ignore the global picture.

\noindent\textbf{Pseudo-code of Cycle-Resemblance Attention Module.} Our proposed cycle-resemblance attention module is shown in {Algorithm}~\ref{algo:cra}.



%说一下原因和结果
%main paper

% The number of blocks is increased from 1 to 9 with a step of 2.



==> z_submission.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{wacv}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{ wasysym }
% \usepackage{multirow}
% \usepackage{multicol}
% \usepackage{caption}
% % Include other packages here, before hyperref.

% \newcommand{\syz}[1]{\textcolor{blue}{#1}}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% %%% IMPORTANT - These next three lines are CRUCIAL.
% %               (1) PLEASE enter your paper ID (given by CMT) replacing the
% %                   '****' right below here with the ID from CMT.
% %               (2) If you are submitting to the Algorithms track, then uncomment
% %                   the \wacvalgorithmstrack line below. If you are submitting to the
% %                   Applications track, then uncomment the \wacvapplicationstrack line.
% %                   If you do not update this properly, we cannot guarantee
% %                   that your paper will be evaluated according to the correct
% %                   review criteria!
% %               (3) Leave the \wacvfinalcopy commented out for the submission
% %                   version, but UNCOMMENT it for your CAMERA-READY upload.
 
% %(1)
% \def\wacvPaperID{1171} % Enter the WACV Paper ID here

% %(2)
% % \wacvalgorithmstrack   % Uncomment this line if you are submitting to the Algorithms Track.
% \wacvapplicationstrack % Uncomment this line if you are submitting to the Applications Track.

% %(3)
% %\wacvfinalcopy % *** Uncomment this line for the final submission
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \ifwacvfinal
% \usepackage[breaklinks=true,bookmarks=false]{hyperref}
% \else
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}
% \fi

% % Pages are numbered in submission mode, and unnumbered in camera-ready
% \pagestyle{empty}

% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% \begin{document}

% %%%%%%%%% TITLE
% \title{Few-shot Medical Image Segmentation with Cycle-resemblance Attention}

% \author{Hao Ding\\
% Illinois Institute of Technology\\
% Institution1 address\\
% {\tt\small hding9@hawk.iit.edu}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }

% \maketitle
% \thispagestyle{empty}


% \input{0_Abstrct}
% \input{1_Introduction.tex}
% \input{2_Related_work.tex}
% \input{3_Proposed_Method.tex}
% \input{4_Experiments.tex}
% \input{5_Conclusion.tex}

% {\small
% \bibliographystyle{ieee_fullname}
% \bibliography{egbib}
% }

% \clearpage
% \setcounter{page}{1}
% \input{6_Supplementary_Materials}
% \end{document}








